Front2Back: Single View 3D Shape Reconstruction via Front to Back Prediction

Reconstruction of a 3D shape from a single 2D image is a classical computer vision problem, whose difficulty stems from the inherent ambiguity of recovering occluded or only partially observed surfaces. Recent methods address this challenge through the use of largely unstructured neural networks that effectively distill conditional mapping and priors over 3D shape. In this work, we induce structure and geometric constraints by leveraging three core observations: (1) the surface of most everyday objects is often almost entirely exposed from pairs of typical opposite views; (2) everyday objects often exhibit global reflective symmetries which can be accurately predicted from single views; (3) opposite orthographic views of a 3D shape share consistent silhouettes. Following these observations, we first predict orthographic 2.5D visible surface maps (depth, normal and silhouette) from perspective 2D images, and detect global reflective symmetries in this data; second, we predict the back facing depth and normal maps using as input the front maps and, when available, the symmetric reflections of these maps; and finally, we reconstruct a 3D mesh from the union of these maps using a surface reconstruction method best suited for this data. Our experiments demonstrate that our framework outperforms state-of-the art approaches for 3D shape reconstructions from 2D and 2.5D data in terms of input fidelity and details preservation. Specifically, we achieve 12% better performance on average in ShapeNet benchmark dataset, and up to 19% for certain classes of objects (e.g., chairs and vessels).

==> text/implementation.tex <==
% \begin{figure*}[th]
%   \centering
%   \includegraphics[width=1.0\textwidth]{figure/overview.png}
%   \caption{{\bf Approach overview.} Our method consists of three steps: (1) Given the front facing normal and depth maps, we first detect the global symmetry plane. With the help of symmetry plane, we can obtain reflected back view maps. (2) We then train an image-to-image translation neural network to predict back view oriented depth maps from the front view maps with reflected maps for reference. (3) The combination of front and back view oriented depth maps provide us a oriented point cloud. Finally we apply Poisson Surface Reconstruction to obtain a watertight 3D mesh.}
%  \label{fig:methodOverview}
% \end{figure*}



\section{Implementation Details}
\label{sec:implementation}

\comment{
\alla{in correct terminology note that we minimize the sum of the loss functions across the three produced maps}
For the 2D to 2.5D step we trained the 2.5D estimation network of \cite{wu2018learning}. The network of  \cite{wu2018learning} is designed for noisy, real-life images and purposefully adds noise to input data to mimic real-life artifacts; since similar to most recent single view reconstruction methods our training image set is synthetic, for a fair comparison we disabled this feature.  We subsequently mask the depth and normal maps using the silhouette map, denoting all pixels outside it as background. 
}

During reflection plane computation we represent each plane $P$ as a 4-dimensional vector $(\alpha_{ij}, \beta_{ij}, \gamma_{ij}, d_{ij})$, where $\alpha_{ij}, \beta_{ij}, \gamma_{ij}$ are the Euler angles of the plane's orientation, and $d_{ij}$ is the distance of the plane to the origin. We define the norm of the 4D vector space of planes as the weighted sum ${\left\lVert (\alpha, \beta, d)\right\rVert}^2 = (w_1\alpha)^2+(w_2\beta)^2+(w_3d)^2$, where the weights for elevation and azimuth angle are $w_1=w_2=\frac{1}{\pi}$ and the distance is weighted by $w_3=0.6\sqrt{2}$. 
RANSAC: sampling 4000 out of about 10000 to 80000 votes, depending on the number of front and back points.
For symmetry detection, we follow the procedure described in Section~\ref{sec:symmetry} and use mean-shift clustering with the Epanechnikov kernel to generate initial symmetry plane guesses. 
% mostly follow the method described in~\cite{mitra2006partial} using mean-shift clustering with the Epanechnikov kernel. 
%After generating the initial guess, we perform a fixed number of optimization iterations. We found that 40 iterations are enough for the models in our test data set to converge to a good solution. Our test set contains both symmetric and asymmetric models; approximately 2\% of the inputs in our test set were not symmetric.
%Each iteration, we firstly compute the pairs of closest points between the original oriented points and reflected ones. The objective function can then be considered as a differentiable function of the symmetry plane as the pairs are fixed. Then we just use gradient decent with backtracking line search for computing the step size.

\alla{is this still accurate?}
To reduce training time, we trained pix2pix~\cite{isola2017image} with the resnet-9 block, instead of pix2pixHD~\cite{wang2017high}, to predict the back view oriented depth maps. Our input images are $256 \times 256$ pixels and have eight channels (three channels for the normals, one channel for the depth; both for front view and reflected view). Our training data set contained the car, airplane, and chair models separately to allow testing on these classes. This is consistent with other papers in the area. We also trained a network with all models to test its performance. 


\comment{
For the final surface reconstruction, we first generate the oriented point cloud by combining the front, reflected, and predicted back maps. Notably for each pixel within the predicted object silhouette we can have either two or three pairs of depth+normal values, one from each map (the reflected map typically covers only a portion of  these pixels, Figure~\ref{fig:reflected}). Basic geometric analysis states that given front and back map depth values for the same pixel a correct front map depth value should always be closer to the observer than the back one. Since back maps are predicted from the front maps, we expect the front prediction to be more accurate.  We consequently ignore back map depth+normal pairs that violate this prior when assembling the point-cloud. We apply a similar logic when assessing consistency between reflected maps and back or front ones. Specifically, since reflected maps are generated from the front ones using well defined priors, we expect front maps to be more reliable than reflected ones, and reflected to be more reliable than back. Consequently given front and reflected map depth values for the same pixel, we ignore reflected map values whenever the reflected depth is closer to the observer than the front one, and given back and reflected map depth values for the same pixel, we ignore back map values whenever the back depth is farther from the observer than the reflected one. 

We subsequently remove outliers from this cloud using the following observation - while we expect our data to contain depth discontinuities we expect prominent features (which have a distinctly different depth than that of their surroundings) to have a front (or back) facing  area bigger than a single pixel. Thus we filter out points if the minimal depth differential between their depth and that of their four immediate neighbors in image space is above a fixed threshold (1.5\% of the image depth range in our implementation \alla{check again the number}).  After that, we use the source code provided by the authors of Poisson surface reconstruction~\cite{kazhdan2013screened} to obtain shape reconstruction result. To allow reconstruction of the details visible in the $256 \times 256$ input images while generating smooth mesh, we set the octree depth of the internal volumetric representation to $7$. \alla{any other parameters?}
}


%where $\Delta_x$ and $\Delta_y$ represent the tangent along the x axis and y axis respectively. $w_x, w_y$ are the Gaussian weights to make sure the constrains are only applied on smooth region. 



%In Computer Graphics, researchers have worked on surface reconstruction from point set for a long time. There are many mature algorithm, such as Marching Cube~\cite{lorensen1987marching}, Poisson Surface Reconstruction~\cite{kazhdan2013screened}, RBF~\cite{carr2001reconstruction} and etc. We observed Poisson Surface Reconstruction~\cite{kazhdan2006poisson} best matches our task as we already have the oriented point cloud. It wants to solve an indicator function $\chi$ which satisfies:
%\begin{equation}
%\chi = \bigg\{ 
%\begin{tabular}{cc}
%0,& outside the model\\
%1,& inside the model
%\end{tabular}
%\end{equation}

%Obviously, the indicator function also gives us the surface of the model. The problem of computing the indicator function can be reduced to approximating the vector field $\overrightarrow{V}$ of the oriented points by the gradient of the function, which is derived as 
%\begin{equation}
%min_{\chi} \left\lVert \nabla\chi - \overrightarrow{V} \right\rVert
%\end{equation}

%This formula can be further cast as a Poisson problem. After solve the Poisson equation, the isosurface is extracted which is the final surface. This method has been demonstrated to generate watertight 3D mesh. 








